The Prefetch Aggressiveness Tradeoff in 360$^{\circ}$ Video Streaming

With 360$^{\circ}$ video, only a limited fraction of the full view is displayed at each point in time. This has prompted the design of streaming delivery techniques that allow alternative playback qualities to be delivered for each candidate viewing direction. However, while prefetching based on the user's expected viewing direction is best done close to playback deadlines, large buffers are needed to protect against shortfalls in future available bandwidth. This results in conflicting goals and an important prefetch aggressiveness tradeoff problem regarding how far ahead in time from the current playpoint prefetching should be done. This paper presents the first characterization of this tradeoff. The main contributions include an empirical characterization of head movement behavior based on data from viewing sessions of four different categories of 360$^{\circ}$ video, an optimization-based comparison of the prefetch aggressiveness tradeoffs seen for these video categories, and a data-driven discussion of further optimizations, which include a novel system design that allows both tradeoff objectives to be targeted simultaneously. By qualitatively and quantitatively analyzing the above tradeoffs, we provide insights into how to best design tomorrow's delivery systems for 360$^{\circ}$ videos, allowing content providers to reduce bandwidth costs and improve users' playback experiences.

==> Makefile <==
all:
	pdflatex tomm-version -dPDFSETTINGS=/prepress
	pdflatex tomm-version -dPDFSETTINGS=/prepress
	bibtex tomm-version
	pdflatex tomm-version -dPDFSETTINGS=/prepress
	pdflatex tomm-version -dPDFSETTINGS=/prepress
	gs -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=letter -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutp\utFile=test.pdf tomm-version.pdf
	mv test.pdf tomm-version.pdf
	cp tomm-version.pdf /wwwpub/nikca89/tmp/paper360.pdf

mmsys:
	pdflatex paper360 -dPDFSETTINGS=/prepress
	pdflatex paper360 -dPDFSETTINGS=/prepress
	bibtex paper360
	pdflatex paper360 -dPDFSETTINGS=/prepress
	pdflatex paper360 -dPDFSETTINGS=/prepress
	#pdflatex lcn -sDEVICE=pdfwrite -sPAPERSIZE=letter -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true
	gs -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=letter -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=test.pdf paper360.pdf
	mv test.pdf paper360.pdf
	cp paper360.pdf /wwwpub/nikca89/tmp/paper360.pdf
#	pdf2ps tatiana.pdf dummy.ps

#niklas:
#	cp tatiana.pdf ~/www-pub/tmp/tatiana.pdf

arxiv:
	pdflatex arxiv-copy
	pdflatex arxiv-copy
	bibtex arxiv-copy
	pdflatex arxiv-copy
	pdflatex arxiv-copy
	gs -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=letter -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=test.pdf arxiv-copy.pdf
	mv test.pdf arxiv-copy.pdf
	cp arxiv-copy.pdf /wwwpub/nikca89/tmp/paper360.pdf


zip-arxiv:
	zip arxiv-copy.zip references.bib arxiv-copy.tex arxiv-copy.pdf arxiv-copy.bbl acmart.cls *.sty arxiv-figs/*.pdf arxiv-figs/*.png Makefile

web:
	pdflatex mmsys18-web -dPDFSETTINGS=/prepress
	pdflatex mmsys18-web -dPDFSETTINGS=/prepress
	bibtex  mmsys18-web
	pdflatex mmsys18-web -dPDFSETTINGS=/prepress
	pdflatex mmsys18-web -dPDFSETTINGS=/prepress
	gs -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=letter -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=test.pdf mmsys18-web.pdf
	mv test.pdf  mmsys18-web.pdf
	cp mmsys18-web.pdf ~/www-pub/tmp/paper360.pdf

zip:
	zip paper360.zip *.tex *.bib *.sty *.cls paper360.pdf figs/*.pdf ../code/charFigs/*.pdf

test:
	echo "blah"

